Using Scene Graph Context to Improve Image Generation

Generating realistic images from scene graphs asks neural networks to be able to reason about object relationships and compositionality. As a relatively new task, how to properly ensure the generated images comply with scene graphs or how to measure task performance remains an open question. In this paper, we propose to harness scene graph context to improve image generation from scene graphs. We introduce a scene graph context network that pools features generated by a graph convolutional neural network that are then provided to both the image generation network and the adversarial loss. With the context network, our model is trained to not only generate realistic looking images, but also to better preserve non-spatial object relationships. We also define two novel evaluation metrics, the relation score and the mean opinion relation score, for this task that directly evaluate scene graph compliance. We use both quantitative and qualitative studies to demonstrate that our pro-posed model outperforms the state-of-the-art on this challenging task.

==> tex/results/old/analysis-results.tex <==
\newcommand{\currsize}{0.21}

\begin{figure*}[!t] \begin{center}
\begin{subfigure}[b]{\currsize\textwidth}
    \includegraphics[width=\textwidth]{images/generic/000017_gt_img.png}
  \end{subfigure}
  \begin{subfigure}[b]{\currsize\textwidth}
    \includegraphics[width=\textwidth]{images/generic/000017_gtb_gtm_img.png}
  \end{subfigure}
  \begin{subfigure}[b]{\currsize\textwidth}
    \includegraphics[width=\textwidth]{images/generic/000017_gtb_pm_img.png}
  \end{subfigure}
  \begin{subfigure}[b]{\currsize\textwidth}
    \includegraphics[width=\textwidth]{images/generic/000017_pred_img.png}
  \end{subfigure}
  \\
\begin{subfigure}[b]{\currsize\textwidth}
    \includegraphics[width=\textwidth]{images/generic/000017_gt_img_updated_updated.png}
  \end{subfigure}
  \begin{subfigure}[b]{\currsize\textwidth}
    \includegraphics[width=\textwidth]{images/generic/000017_gtb_gtm_img_updated_updated.png}
  \end{subfigure}
  \begin{subfigure}[b]{\currsize\textwidth}
    \includegraphics[width=\textwidth]{images/generic/000017_gtb_pm_img_updated_updated.png}
  \end{subfigure}
  \begin{subfigure}[b]{\currsize\textwidth}
    \includegraphics[width=\textwidth]{images/generic/000017_pred_img_updated_updated.png}
  \end{subfigure}
\\
\begin{subfigure}[b]{\currsize\textwidth}
    \includegraphics[width=\textwidth]{images/generic/000025_gt_img.png}
  \end{subfigure}
  \begin{subfigure}[b]{\currsize\textwidth}
    \includegraphics[width=\textwidth]{images/generic/000025_gtb_gtm_img.png}
  \end{subfigure}
  \begin{subfigure}[b]{\currsize\textwidth}
    \includegraphics[width=\textwidth]{images/generic/000025_gtb_pm_img.png}
  \end{subfigure}
  \begin{subfigure}[b]{\currsize\textwidth}
    \includegraphics[width=\textwidth]{images/generic/000025_pred_img.png}
  \end{subfigure}
  \\
\begin{subfigure}[b]{\currsize\textwidth}
    \includegraphics[width=\textwidth]{images/generic/000025_gt_img_updated_updated.png}
  \end{subfigure}
  \begin{subfigure}[b]{\currsize\textwidth}
    \includegraphics[width=\textwidth]{images/generic/000025_gtb_gtm_img_updated_updated.png}
  \end{subfigure}
  \begin{subfigure}[b]{\currsize\textwidth}
    \includegraphics[width=\textwidth]{images/generic/000025_gtb_pm_img_updated_updated.png}
  \end{subfigure}
  \begin{subfigure}[b]{\currsize\textwidth}
    \includegraphics[width=\textwidth]{images/generic/000025_pred_img_updated_updated.png}
  \end{subfigure}
  \\
\begin{subfigure}[b]{\currsize\textwidth}
    \includegraphics[width=\textwidth]{images/generic/000088_gt_img.png}
  \end{subfigure}
  \begin{subfigure}[b]{\currsize\textwidth}
    \includegraphics[width=\textwidth]{images/generic/000088_gtb_gtm_img.png}
  \end{subfigure}
  \begin{subfigure}[b]{\currsize\textwidth}
    \includegraphics[width=\textwidth]{images/generic/000088_gtb_pm_img.png}
  \end{subfigure}
  \begin{subfigure}[b]{\currsize\textwidth}
    \includegraphics[width=\textwidth]{images/generic/000088_pred_img.png}
  \end{subfigure}
  \\
\begin{subfigure}[b]{\currsize\textwidth}
    \includegraphics[width=\textwidth]{images/generic/000088_gt_img_updated_updated.png}
        \caption{Ground truth}
    \label{fig_1:1}
  \end{subfigure}
  \begin{subfigure}[b]{\currsize\textwidth}
    \includegraphics[width=\textwidth]{images/generic/000088_gtb_gtm_img_updated_updated.png}
        \caption{GT Box, GT mask}
    \label{fig_1:2}
  \end{subfigure}
  \begin{subfigure}[b]{\currsize\textwidth}
    \includegraphics[width=\textwidth]{images/generic/000088_gtb_pm_img_updated_updated.png}
        \caption{GT Box, pred mask}
    \label{fig_1:3}
  \end{subfigure}
  \begin{subfigure}[b]{\currsize\textwidth}
    \includegraphics[width=\textwidth]{images/generic/000088_pred_img_updated_updated.png}
        \caption{All predicted}
    \label{fig_1:4}
  \end{subfigure}
\caption{Images generated with available ground truth box and mask}  
\label{fig:result_analysis1}
\end{center}\end{figure*}





\begin{figure*}[!t] \begin{center}
\begin{subfigure}[b]{\currsize\textwidth}
    \includegraphics[width=\textwidth]{images/generic/000119_gt_img.png}
  \end{subfigure}
  \begin{subfigure}[b]{\currsize\textwidth}
    \includegraphics[width=\textwidth]{images/generic/000119_gtb_gtm_img.png}
  \end{subfigure}
  \begin{subfigure}[b]{\currsize\textwidth}
    \includegraphics[width=\textwidth]{images/generic/000119_gtb_pm_img.png}
  \end{subfigure}
  \begin{subfigure}[b]{\currsize\textwidth}
    \includegraphics[width=\textwidth]{images/generic/000119_pred_img.png}
  \end{subfigure}
  \\
\begin{subfigure}[b]{\currsize\textwidth}
    \includegraphics[width=\textwidth]{images/generic/000119_gt_img_updated_updated.png}
  \end{subfigure}
  \begin{subfigure}[b]{\currsize\textwidth}
    \includegraphics[width=\textwidth]{images/generic/000119_gtb_gtm_img_updated_updated.png}
  \end{subfigure}
  \begin{subfigure}[b]{\currsize\textwidth}
    \includegraphics[width=\textwidth]{images/generic/000119_gtb_pm_img_updated_updated.png}
  \end{subfigure}
  \begin{subfigure}[b]{\currsize\textwidth}
    \includegraphics[width=\textwidth]{images/generic/000119_pred_img_updated_updated.png}
  \end{subfigure}
  \\
  \begin{subfigure}[b]{\currsize\textwidth}
    \includegraphics[width=\textwidth]{images/generic/000245_gt_img.png}
  \end{subfigure}
  \begin{subfigure}[b]{\currsize\textwidth}
    \includegraphics[width=\textwidth]{images/generic/000245_gtb_gtm_img.png}
  \end{subfigure}
  \begin{subfigure}[b]{\currsize\textwidth}
    \includegraphics[width=\textwidth]{images/generic/000245_gtb_pm_img.png}
  \end{subfigure}
  \begin{subfigure}[b]{\currsize\textwidth}
    \includegraphics[width=\textwidth]{images/generic/000245_pred_img.png}
  \end{subfigure}
  \\
\begin{subfigure}[b]{\currsize\textwidth}
    \includegraphics[width=\textwidth]{images/generic/000245_gt_img_updated_updated.png}
  \end{subfigure}
  \begin{subfigure}[b]{\currsize\textwidth}
    \includegraphics[width=\textwidth]{images/generic/000245_gtb_gtm_img_updated_updated.png}
  \end{subfigure}
  \begin{subfigure}[b]{\currsize\textwidth}
    \includegraphics[width=\textwidth]{images/generic/000245_gtb_pm_img_updated_updated.png}
  \end{subfigure}
  \begin{subfigure}[b]{\currsize\textwidth}
    \includegraphics[width=\textwidth]{images/generic/000245_pred_img_updated_updated.png}
  \end{subfigure}
  \\
  \\
  \begin{subfigure}[b]{\currsize\textwidth}
    \includegraphics[width=\textwidth]{images/generic/000780_gt_img.png}
  \end{subfigure}
  \begin{subfigure}[b]{\currsize\textwidth}
    \includegraphics[width=\textwidth]{images/generic/000780_gtb_gtm_img.png}
  \end{subfigure}
  \begin{subfigure}[b]{\currsize\textwidth}
    \includegraphics[width=\textwidth]{images/generic/000780_gtb_pm_img.png}
  \end{subfigure}
  \begin{subfigure}[b]{\currsize\textwidth}
    \includegraphics[width=\textwidth]{images/generic/000780_pred_img.png}
  \end{subfigure}
  \\
\begin{subfigure}[b]{\currsize\textwidth}
    \includegraphics[width=\textwidth]{images/generic/000780_gt_img_updated_updated.png}
    \caption{Ground truth}
    \label{fig_2:1}
  \end{subfigure}
  \begin{subfigure}[b]{\currsize\textwidth}
    \includegraphics[width=\textwidth]{images/generic/000780_gtb_gtm_img_updated_updated.png}
    \caption{GT Box, GT Mask}
    \label{fig_2:2}
  \end{subfigure}
  \begin{subfigure}[b]{\currsize\textwidth}
    \includegraphics[width=\textwidth]{images/generic/000780_gtb_pm_img_updated_updated.png}
        \caption{GT Box, pred Mask}
    \label{fig_2:3}
  \end{subfigure}
  \begin{subfigure}[b]{\currsize\textwidth}
    \includegraphics[width=\textwidth]{images/generic/000780_pred_img_updated_updated.png}
    \caption{All predicted}
    \label{fig_2:4}
  \end{subfigure}
  \caption{Images generated with available ground truth box and mask}  
\label{fig:result_analysis2}
\end{center}\end{figure*}

==> tex/results/old/attribute-results.tex <==
\newcommand{\currsizeat}{0.25}

\begin{figure*}[!t] \begin{center}
\begin{subfigure}[b]{\currsizeat\textwidth}
    \includegraphics[width=\textwidth]{images/attributes/000164_gt_img.png}
  \end{subfigure}
  %
  \begin{subfigure}[b]{\currsizeat\textwidth}
    \includegraphics[width=\textwidth]{images/attributes/000164_pred_img.png}
  \end{subfigure}
  \begin{subfigure}[b]{\currsizeat\textwidth}
    \includegraphics[width=\textwidth]{images/attributes/000164_pred_img_updated.png}
  \end{subfigure}
  \\
\begin{subfigure}[b]{\currsizeat\textwidth}
    \includegraphics[width=\textwidth]{images/attributes/000757_gt_img.png}
    \caption{Ground Truth}
    \label{fig_3:1}
  \end{subfigure}
  %
  \begin{subfigure}[b]{\currsizeat\textwidth}
    \includegraphics[width=\textwidth]{images/attributes/000757_pred_img.png}
    \caption{SG2Im results}
    \label{fig_3:2}
  \end{subfigure}
  \begin{subfigure}[b]{\currsizeat\textwidth}
    \includegraphics[width=\textwidth]{images/attributes/000757_pred_img_updated.png}
    \caption{Scene context Results}
    \label{fig_3:3}
  \end{subfigure}

\caption{Need to incorporate attributes in the Graph convolutional network}  
\label{fig:result_attributes}
\end{center}\end{figure*}

==> tex/results/old/failure-results.tex <==
\newcommand{\currsizef}{0.25}

\begin{figure*}[!t] \begin{center}
\begin{subfigure}[b]{\currsizef\textwidth}
    \includegraphics[width=\textwidth]{images/failure/000118_gt_img.png}
  \end{subfigure}
  %
  \begin{subfigure}[b]{\currsizef\textwidth}
    \includegraphics[width=\textwidth]{images/failure/000118_pred_img.png}
  \end{subfigure}
  \begin{subfigure}[b]{\currsizef\textwidth}
    \includegraphics[width=\textwidth]{images/failure/000118_pred_img_updated.png}
  \end{subfigure}
  \\
\begin{subfigure}[b]{\currsizef\textwidth}
    \includegraphics[width=\textwidth]{images/failure/000471_gt_img.png}
  \end{subfigure}
  %
  \begin{subfigure}[b]{\currsizef\textwidth}
    \includegraphics[width=\textwidth]{images/failure/000471_pred_img.png}
  \end{subfigure}
  \begin{subfigure}[b]{\currsizef\textwidth}
    \includegraphics[width=\textwidth]{images/failure/000471_pred_img_updated.png}
  \end{subfigure}
  \\
  \begin{subfigure}[b]{\currsizef\textwidth}
    \includegraphics[width=\textwidth]{images/failure/000632_gt_img.png}
  \end{subfigure}
  \begin{subfigure}[b]{\currsizef\textwidth}
    \includegraphics[width=\textwidth]{images/failure/000632_pred_img.png}
  \end{subfigure}
  \begin{subfigure}[b]{\currsizef\textwidth}
    \includegraphics[width=\textwidth]{images/failure/000632_pred_img_updated.png}
  \end{subfigure}
  \\
  \begin{subfigure}[b]{\currsizef\textwidth}
    \includegraphics[width=\textwidth]{images/failure/000790_gt_img.png}
  \end{subfigure}
  \begin{subfigure}[b]{\currsizef\textwidth}
    \includegraphics[width=\textwidth]{images/failure/000790_pred_img.png}
  \end{subfigure}
  \begin{subfigure}[b]{\currsizef\textwidth}
    \includegraphics[width=\textwidth]{images/failure/000790_pred_img_updated.png}
  \end{subfigure}
  \\
\begin{subfigure}[b]{\currsizef\textwidth}
    \includegraphics[width=\textwidth]{images/failure/000816_gt_img.png}
    \caption{Ground Truth}
    \label{fig_4:1}
  \end{subfigure}
  \begin{subfigure}[b]{\currsizef\textwidth}
    \includegraphics[width=\textwidth]{images/failure/000816_pred_img.png}
    \caption{SG2Im results}
    \label{fig_4:2}
  \end{subfigure}
  \begin{subfigure}[b]{\currsizef\textwidth}
    \includegraphics[width=\textwidth]{images/failure/000816_pred_img_updated.png}
    \caption{scene-context results}
    \label{fig_4:3}
  \end{subfigure}

\caption{Failure cases for the scenegraph context model}  
\label{fig:result_failure}
\end{center}\end{figure*}

==> tex/results/old/similarity-results.tex <==
\newcommand{\mysizes}{0.3}

\begin{figure*}[!t] \begin{center}
\begin{subfigure}[b]{\mysizes\textwidth}
    \includegraphics[width=\textwidth]{images/same/000270_gt_img.png}
  \end{subfigure}
  %
  \begin{subfigure}[b]{\mysizes\textwidth}
    \includegraphics[width=\textwidth]{images/same/000270_pred_img.png}
  \end{subfigure}
  \begin{subfigure}[b]{\mysizes\textwidth}
    \includegraphics[width=\textwidth]{images/same/000270_pred_img_updated.png}
  \end{subfigure}
  \\
\begin{subfigure}[b]{\mysizes\textwidth}
    \includegraphics[width=\textwidth]{images/same/000727_gt_img.png}
  \end{subfigure}
  %
  \begin{subfigure}[b]{\mysizes\textwidth}
    \includegraphics[width=\textwidth]{images/same/000727_pred_img.png}
  \end{subfigure}
  \begin{subfigure}[b]{\mysizes\textwidth}
    \includegraphics[width=\textwidth]{images/same/000727_pred_img_updated.png}
  \end{subfigure}
  \\
\begin{subfigure}[b]{\mysizes\textwidth}
    \includegraphics[width=\textwidth]{images/same/000976_gt_img.png}
    \caption{Ground Truth}
    \label{fig_5:1}
  \end{subfigure}
  %
  \begin{subfigure}[b]{\mysizes\textwidth}
    \includegraphics[width=\textwidth]{images/same/000976_pred_img.png}
    \caption{SG2Im results}
    \label{fig_5:2}
  \end{subfigure}
  \begin{subfigure}[b]{\mysizes\textwidth}
    \includegraphics[width=\textwidth]{images/same/000976_pred_img_updated.png}
    \caption{scene context results}
    \label{fig_5:3}
  \end{subfigure}

\caption{scene-context results}  
\label{fig:result_similar}
\end{center}\end{figure*}

==> tex/results/visual_comparison_vg.tex <==
\newcommand{\vgs}{0.18}

\begin{figure*}[!t] \begin{center}
\begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/sgc/000180_sg.png}
  \end{subfigure}
  \begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/sgc/000180_pred_img.png}
  \end{subfigure}
  \begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/sgc/000180_gtb_pm_img.png}
  \end{subfigure}
\begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/jj/000180_gt_img.png}
  \end{subfigure}
  
\begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/gt/000180_sg.png}
  \end{subfigure}
  \begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/jj/000180_pred_img.png}
  \end{subfigure}
  \begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/jj/000180_gtb_pm_img.png}
  \end{subfigure}
\begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/jj/000180_gt_img.png}
  \end{subfigure}
   \vspace{3.00mm}
      
      
\begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/gt/000346_sg.png}
  \end{subfigure}
  \begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/sgc/000346_pred_img.png}
  \end{subfigure}
  \begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/sgc/000346_gtb_pm_img.png}
  \end{subfigure}
\begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/jj/000346_gt_img.png}
  \end{subfigure}
  
\begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/gt/000346_sg.png}
  \end{subfigure}
  \begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/jj/000346_pred_img.png}
  \end{subfigure}
  \begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/jj/000346_gtb_pm_img.png}
  \end{subfigure}
\begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/jj/000346_gt_img.png}
  \end{subfigure}
   \vspace{3.00mm}

\begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/gt/000551_sg.png}
  \end{subfigure}
  \begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/sgc/000551_pred_img.png}
  \end{subfigure}
  \begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/sgc/000551_gtb_pm_img.png}
  \end{subfigure}
\begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/jj/000551_gt_img.png}
  \end{subfigure}
  
\begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/gt/000551_sg.png}
        \caption{Input scenegraph}
  \end{subfigure}
  \begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/jj/000551_pred_img.png}
        \caption{Generated image}
  \end{subfigure}
  \begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/jj/000551_gtb_pm_img.png}
        \caption{with GT box}
  \end{subfigure}
\begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/jj/000551_gt_img.png}
    \caption{Ground truth}
  \end{subfigure}
   \vspace{3.00mm}
   
\caption{Sample results of generated images, image generated with ground truth boxes and ground truth images corresponding to for query scenegraphs from visual genome test set. Top row corresponds to scene-context network results and bottom row corresponds to \cite{img_gen_from_scene_graph18} for every pair of rows. In general scene-context helps in better layout prediction and pixel generation.}  
\label{fig:visual1}
\end{center}\end{figure*}




\begin{figure*}[!t] \begin{center}
\begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/gt/000649_sg.png}
  \end{subfigure}
  \begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/sgc/000649_pred_img.png}
  \end{subfigure}
  \begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/sgc/000649_gtb_pm_img.png}
  \end{subfigure}
\begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/jj/000649_gt_img.png}
  \end{subfigure}
  
\begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/gt/000649_sg.png}
  \end{subfigure}
  \begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/jj/000649_pred_img.png}
  \end{subfigure}
  \begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/jj/000649_gtb_pm_img.png}
  \end{subfigure}
\begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/jj/000649_gt_img.png}
  \end{subfigure}
   \vspace{3.00mm}
      
\begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/gt/000715_sg.png}
  \end{subfigure}
  \begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/sgc/000715_pred_img.png}
  \end{subfigure}
  \begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/sgc/000715_gtb_pm_img.png}
  \end{subfigure}
\begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/jj/000715_gt_img.png}
  \end{subfigure}
  
\begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/gt/000715_sg.png}
  \end{subfigure}
  \begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/jj/000715_pred_img.png}
  \end{subfigure}
  \begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/jj/000715_gtb_pm_img.png}
  \end{subfigure}
\begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/jj/000715_gt_img.png}
  \end{subfigure}
   \vspace{3.00mm}

\begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/gt/000920_sg.png}
  \end{subfigure}
  \begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/sgc/000920_pred_img.png}
  \end{subfigure}
  \begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/sgc/000920_gtb_pm_img.png}
  \end{subfigure}
\begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/jj/000920_gt_img.png}
  \end{subfigure}
  
\begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/gt/000920_sg.png}
    \caption{Input SceneGraph}
  \end{subfigure}
  \begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/jj/000920_pred_img.png}
    \caption{Generated image}
  \end{subfigure}
  \begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/jj/000920_gtb_pm_img.png}
    \caption{with GT box}
  \end{subfigure}
\begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/jj/000920_gt_img.png}
        \caption{Ground truth}
  \end{subfigure}
   \vspace{3.00mm}
   
\caption{Sample results of generated images, image generated with ground truth boxes and ground truth images corresponding to for query scenegraphs from visual genome test set. Top row corresponds to scene-context network results and bottom row corresponds to \cite{img_gen_from_scene_graph18} for every pair of rows. In general scene-context helps in better layout prediction and pixel generation.}  
\label{fig:visual1}
\end{center}\end{figure*}


\begin{figure*}[!t] \begin{center}
\begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/gt/001005_sg.png}
  \end{subfigure}
  \begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/sgc/001005_pred_img.png}
  \end{subfigure}
  \begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/sgc/001005_gtb_pm_img.png}
  \end{subfigure}
\begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/jj/001005_gt_img.png}
  \end{subfigure}
  
\begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/gt/001005_sg.png}
  \end{subfigure}
  \begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/jj/001005_pred_img.png}
  \end{subfigure}
  \begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/jj/001005_gtb_pm_img.png}
  \end{subfigure}
\begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/jj/001005_gt_img.png}
  \end{subfigure}
   \vspace{3.00mm}
      
% % \begin{subfigure}[b]{\vgs\textwidth}
% %     \includegraphics[width=\textwidth]{images/coco/000028_layout.png}
% %   \end{subfigure}
%   \begin{subfigure}[b]{\vgs\textwidth}
%     \includegraphics[width=\textwidth]{images/vg/sgc/001019_pred_img.png}
%   \end{subfigure}
%   \begin{subfigure}[b]{\vgs\textwidth}
%     \includegraphics[width=\textwidth]{images/vg/sgc/001019_gtb_pm_img.png}
%   \end{subfigure}
% \begin{subfigure}[b]{\vgs\textwidth}
%     \includegraphics[width=\textwidth]{images/vg/jj/001019_gt_img.png}
%   \end{subfigure}
  
% %   \begin{subfigure}[b]{\vgs\textwidth}
% %     \includegraphics[width=\textwidth]{images/coco/000028_layout_jj.png}
% %   \end{subfigure}
%   \begin{subfigure}[b]{\vgs\textwidth}
%     \includegraphics[width=\textwidth]{images/vg/jj/001019_pred_img.png}
%   \end{subfigure}
%   \begin{subfigure}[b]{\vgs\textwidth}
%     \includegraphics[width=\textwidth]{images/vg/jj/001019_gtb_pm_img.png}
%   \end{subfigure}
% \begin{subfigure}[b]{\vgs\textwidth}
%     \includegraphics[width=\textwidth]{images/vg/jj/001019_gt_img.png}
%   \end{subfigure}
%   \vspace{3.00mm}
   
   
\begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/gt/001022_sg.png}
  \end{subfigure}
  \begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/sgc/001022_pred_img.png}
  \end{subfigure}
  \begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/sgc/001022_gtb_pm_img.png}
  \end{subfigure}
\begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/jj/001022_gt_img.png}
  \end{subfigure}
  
\begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/gt/001022_sg.png}
  \end{subfigure}
  \begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/jj/001022_pred_img.png}
  \end{subfigure}
  \begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/jj/001022_gtb_pm_img.png}
  \end{subfigure}
\begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/jj/001022_gt_img.png}
  \end{subfigure}
   \vspace{3.00mm}
   

\begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/gt/001020_sg.png}
  \end{subfigure}
  \begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/sgc/001020_pred_img.png}
  \end{subfigure}
  \begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/sgc/001020_gtb_pm_img.png}
  \end{subfigure}
\begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/jj/001020_gt_img.png}
  \end{subfigure}
  
\begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/gt/001020_sg.png}
    \caption{Input scenegraph}
  \end{subfigure}
  \begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/jj/001020_pred_img.png}
    \caption{Generated image}
  \end{subfigure}
  \begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/jj/001020_gtb_pm_img.png}
    \caption{with GT box}
  \end{subfigure}
\begin{subfigure}[b]{\vgs\textwidth}
    \includegraphics[width=\textwidth]{images/vg/jj/001020_gt_img.png}
    \caption{Ground truth}
  \end{subfigure}
   \vspace{3.00mm}
   
\caption{Sample results of generated images, image generated with ground truth boxes and ground truth images corresponding to for query scenegraphs from visual genome test set. Top row corresponds to scene-context network results and bottom row corresponds to \cite{img_gen_from_scene_graph18} for every pair of rows. In general scene-context helps in better layout prediction and pixel generation.}  
\label{fig:visual3}
\end{center}\end{figure*}

